OSR-ViT: A Simple and Modular Framework for Open-Set Object Detection and Discovery

An object detector's ability to detect and flag \textit{novel} objects during open-world deployments is critical for many real-world applications. Unfortunately, much of the work in open object detection today is disjointed and fails to adequately address applications that prioritize unknown object recall \textit{in addition to} known-class accuracy. To close this gap, we present a new task called Open-Set Object Detection and Discovery (OSODD) and as a solution propose the Open-Set Regions with ViT features (OSR-ViT) detection framework. OSR-ViT combines a class-agnostic proposal network with a powerful ViT-based classifier. Its modular design simplifies optimization and allows users to easily swap proposal solutions and feature extractors to best suit their application. Using our multifaceted evaluation protocol, we show that OSR-ViT obtains performance levels that far exceed state-of-the-art supervised methods. Our method also excels in low-data settings, outperforming supervised baselines using a fraction of the training data.

==> sections/old_related_work.tex <==
\section{Limitations of Existing Work}
\frank{Reorganzie this section based on oure discussion: 1) FG/BG distinction 2) FG ID/OOD classification 3) FG OOD classification (open/close vocabulary)}
\label{sec:related_work}



A major limitation of existing ``open'' object detection literature is the incongruity of task goals. The evaluation protocols used in different works vary significantly, making it very challenging to directly compare methods. The reason for this discrepancy is that the ``correct'' way of handling of OOD objects during deployment is subjective and can vary depending on the application. In our estimation, there are currently six main subdivisions that fall under the umbrella of ``open'' object detection that have unique philosophies and goals:

\textbf{Object Discovery (ObjDisc)}. Object discovery models separate objects from background without supervision \cite{OGObjectDiscovery}. These works typically use precision and recall as performance metrics. Early works in this area identify salient regions with respect to image transformations \cite{OGObjectDiscovery, ObjectDiscoveryInTheWild} or noise \cite{ObjectDiscoveryRGBD}. More recent works leverage convolutional features instead of the images directly \cite{DissimilarityCoeffBasedObjDiscovery, ObjectCentricLearningSlotAttention}.

\textbf{Open-World Object Proposal (OWP)}. Class-agnostic object proposal networks seek to maximize ID and OOD object recall \cite{KevinsPaper, OLN, LearningToDetectEveryThing, THPN}. These works use Average Recall (AR) \cite{AverageRecall} as the primary performance metric. Kim et al. \cite{OLN} showed that standard object proposal networks such as Region Proposal Network (RPN) \cite{FasterRCNN} and its variants \cite{CascadeRPN, RegionProposalGuidedAnchoring} overfit to the ID categories because of its discriminative learning approach. They instead propose an Object Localization Network (OLN) which replaces the classification heads of a class-agnostic Faster R-CNN \cite{FasterRCNN} with localization-quality prediction heads, yielding a model that more readily generalizes to OOD objects. Konan et al. \cite{KevinsPaper} use unknown object masking to create a one-stage model that can rival the more powerful two-stage models. Finally, Saito et al. \cite{LearningToDetectEveryThing} use a background erasing augmentation strategy to further reduce the bias of classification-based proposal networks. While class-agnostic detection is useful, class separation is often necessary.

\textbf{Open-Set Object Detection (OSOD)}. An OSOD detector should ignore OOD objects and not let the presence of OOD or ``wilderness'' data effect ID accuracy \cite{OverlookedElephantOpenSet, Miller1, Miller2, Miller3, ExpandingLowDensityLatentRegionsOSOD}. In other words, the goal is to simply avoid mistaking OOD objects as ID classes. OSOD performance is measured by two metrics: (1) Absolute Open Set Error (A-OSE): the total number of OOD instances detected as one of the ID classes \cite{Miller1}, and (2) Wilderness Impact: the ratio of ID precision before and after adding OOD ``wilderness'' data \cite{OverlookedElephantOpenSet}. 
Miller et al. \cite{Miller1} first introduce the notion of open-set object detection and use dropout sampling \cite{DropoutSampling} to improve label uncertainty.
Dhamija et al. \cite{OverlookedElephantOpenSet} show that closed-set detectors tend to misclassify OOD objects as ID classes. 
%Miller et al. \cite{Miller2} investigate other samping-based merging strategies beyond dropout sampling. 
Recently, Han et al. \cite{ExpandingLowDensityLatentRegionsOSOD} use a contrastive feature learner to identify OOD objects from their latent representations. The limitation of OSOD is that the recall of OOD objects is irrelevant, which is unacceptable for many real-world applications (see Fig. \ref{fig:evaluation_viz}).
    
\textbf{Unknown-Aware Object Detection (UAOD)}. An UAOD model should maximize ID performance and precisely flag any OOD objects that happen to be proposed to the classifier head \cite{VOS, SIREN, STUD}. Here, performance is measured by two metrics: (1) ID mean Average Precision (ID mAP) \cite{RCNN}, and (2) the area under the receiver operating characteristic of the binary ID vs. OOD classification component (i.e., ID vs. OOD AUROC) \cite{MSP}.
%These works require two different validation sets: one that contains ID objects (ID-set) and one that is assured to not contain any ID objects (OOD-set). The trained detector then runs inference on both sets and all detections with a maximum (non-background) confidence over a certain threshold are assumed to be valid ID and OOD objects, respectively. This is flawed because even with a good detector, many high-confidence detections are false positives on background regions. Also, there could be valid OOD objects in the ID-set which, if predicted confidently enough, will incorrectly be treated as valid ID predictions during evaluation. 
Du et al. \cite{VOS} generate near-OOD virtual outliers to learn more compact ID clusters to ease the separation of ID and OOD objects. SIREN \cite{SIREN} maps ID-class representations onto a von Mises-Fisher (vMF) distribution to provide a powerful distance-based OOD detection method for detectors. Finally, STUD \cite{STUD} distills unknown objects from video data to improve OOD detection in object detection models.
A major limitation of this subdivision is that most works \cite{VOS, SIREN, STUD} make several unrealistic and invalid assumptions to compute the AUROC metric in a detection task. For example, they require mutually exclusive ID and OOD validation sets, and incorrectly assume that all detections with confidence over a certain threshold are valid ID and OOD predictions, respectively. 
Also, like in OSOD, recall on OOD objects is not measured or prioritized in this task, limiting its practical usefulness. 

\textbf{Open-World Object Detection (OWOD)}. An OWOD detector's goal is to maximize ID performance while also flagging OOD objects. Critically, open-world models also incrementally learn new classes after forwarding the OOD detections to a human-in-the-loop for labeling \cite{TowardsOpenWorldObjectDetection, OWDETR, RevisitingOWOD, UCOWOD, ObjectsInSemanticTopology, OWODDiscriminativeClassPrototype, TwoBranchObjCentricOWOD, PROB}. Most open world detection models use ID mAP and OOD recall (on a set of successive tasks) to measure performance. Joseph et al.'s ORE model \cite{TowardsOpenWorldObjectDetection} uses a conventional RPN with a contrastive clustering regularization to create a baseline. Gupta et al. \cite{OWDETR} introduce a DETR-based \cite{DETR, DeformableDETR} OW-DETR model that boosts performance via attention-driven pseudo-labeling. Wu et al. \cite{TwoBranchObjCentricOWOD} propose a two-branch objectness-centric model that leverages the benefits of OLN's localization-quality prediction head to improve object recall. Finally, Zohar et al.'s PROB model \cite{PROB} specifically addresses unknown object recall with an additional probabilistic objectness head.
While the incremental learning aspect of the OWOD task is interesting, there are many outside factors (e.g., threshold choice, semantic drift between tasks, training data quality) that contribute heavily to perceived performance that it is difficult to judge a model's true usability.
%In our view, the most important component to OWOD is the model's ability to balance ID and OOD detection. Everything else is highly application-specific problem.

\textbf{Open-Vocabulary Object Detection (OVOD)}. An OVOD model uses natural language models to enable the detector to directly generalize beyond the ID classes using text prompting \cite{OVODusingCaptions, OVDETR, ObjectCentricOVD, CORA, ScalingOVOD}. While these approaches are powerful under certain circumstances (i.e., where object classes of interest are well-represented in language datasets), their practical usefulness is limited in many domains (i.e., fine-grained ship detection). In this work, we do not consider OVOD baselines as they lie in a very different multi-modal domain.

